Boundary-weighted logit consistency improves calibration of segmentation networks

Neural network prediction probabilities and accuracy are often only weakly-correlated. Inherent label ambiguity in training data for image segmentation aggravates such miscalibration. We show that logit consistency across stochastic transformations acts as a spatially varying regularizer that prevents overconfident predictions at pixels with ambiguous labels. Our boundary-weighted extension of this regularizer provides state-of-the-art calibration for prostate and heart MRI segmentation.

==> 1_intro_neel.tex <==
% =========================================================
% Introduction
% =========================================================
\section{Introduction}~\label{sec_intro}

\noindent Supervised deep neural networks are susceptible to overfitting on sparsely-labelled training datasets. Data augmentation (DA) tackles this issue by applying task-informed transformations to labelled input-output pairs to expand the training dataset.
Recent work in semi-supervised learning \cite{bortsova2019semi,li2020transformation} extends this idea by formulating unsupervised regularizers that encourage task-specific empirical invariance or equivariance in network predictions on unlabelled images during training.
As these regularizers encourage consistent predictions across transformations, we refer to this family of methods as consistency regularization (CR).

\vspace{2pt} \noindent 
While previous work uses CR as a means to learn from unlabelled images, we show that \emph{even without any additional unlabelled images}, CR improves segmentation calibration \cite{guo2017calibration}, and sometimes, even segmentation \emph{accuracy} of neural networks over those trained with DA.
This is surprising as CR does not have access to additional data when employed in the supervised-only setting as compared to DA.
What are the causes of this benefit?

\vspace{2pt} \noindent 
To answer this question, we note that anatomical boundaries are often ambiguous in medical images due to the absence of sufficient contrast, inter-annotator variability, and the presence of noise and/or partial voluming.
% Additionally, annotations from multiple clinical experts exhibit substantial variability \cite{becker2019variability}, leading to further ambiguity in what can be considered as \emph{ground truth} labels \cite{jacob2021disentangling}.
However, common segmentation datasets typically assign \textit{hard} classes for each pixel, thus removing sources of ambiguity.
Supervised learning then insists on exact pixel-wise agreement between predictions and ground truth labels, which can be achieved by over-parameterized neural networks.
For instance, using the cross-entropy loss function for training maximizes logit differences between the ground truth class and other classes for each pixel \cite{murugesan2022calibrating}.
This bias towards low-entropy predictions caused by supervised learning loss functions coupled with the inherent ambiguity in the true underlying labels leads to over-confident predictions and miscalibrated models.

\vspace{2pt} \noindent
Consequently, we speculate that reduced logit differences across classes for pixels with ambiguous labels may counter such miscalibration.
% In the absence of explicit information about label ambiguity in the available annotations, it is unclear how to design loss functions that encourage such behaviour.
Based on this, our paper makes two main contributions.
First, we show that CR can automatically discover such pixels and prevent overfitting to their \emph{noisy} labels.
In doing so, it enforces a spatially varying pixel-wise regularization effect, leading to improved calibration.
In contrast to previous usages of CR in medical image segmentation, the newly discovered benefits in our work are independent of additional unlabelled images.
% To our knowledge, this understanding of CR as well as the connection between the literature on semi-supervised learning and that on segmentation label ambiguity is novel.
% this understanding is novel
% connection between CR, small datasets stuff and label ambiguity is novel.
% using this understanding to further improve the method.
Second, given an understanding of the mechanism underlying the calibration benefits of CR, we propose a spatially-varying weighting strategy for the CR loss relative to the supervised loss.
This strategy emphasizes regularization in pixels near anatomical boundaries, as these pixels are more likely to suffer from label ambiguity.
With the proposed boundary-weighted CR, we demonstrate state-of-the-art calibration in the segmentation of prostate and heart MRI.
Our code will be publicly released.

% noisy labels
% links to label smoothing, spatially varying label smoothing, entropy maximization, margin based calibration methods
% \vspace{5pt} \noindent A problem that is typically considered in isolation from the small-labelled-datasets problem is that of ambiguity in segmentation labels. This arises from the fact that boundaries between anatomical regions are often ambiguous in medical images due to presence of image noise or absence of sufficient contrast. This issue may be exacerbated by partial volume effects~\cite{tohka2014partial}. Additionally, inter-expert preferences lead to further ambiguity in what can be considered as 'ground truth' labels~\cite{jacob2021disentangling}. Supervised learning that does not account for such label ambiguity insists on perfect agreement at every pixel between predictions and ground truth labels, which can be achieved by over-parameterized neural networks and may contribute to overfitting while training with small labelled datasets.
% We hypothesize that this is one of the factors responsible for overfitting while training with small labelled datasets.

% contributions
% \vspace{5pt} \noindent We empirically show that CR achieves these benefits by enforcing a spatially varying pixel-wise regularization effect that prevents overfitting to pixels with ambiguous labels. Endowed with this new understanding of the mechanism underlying the benefits of CR, we propose a spatially-varying weighing strategy for the unsupervised CR loss which emphasizes the regularization loss term in pixels with higher label ambiguity.

% Among reasons for this overfitting behaviour is the existence of spurious correlations between training inputs and outputs, and minimizing solely supervised objectives encourages these spurious correlations to be exploited. Although, it has been shown that networks tend to learn signal before they learn noise.

% list cr approaches
% copy sentences from those papers where they state their motivation

% stress that the main motivation is to utilize unlabelled data

% here, we present a loss landspace perspective of 

% nns can overfit when training datsets are small
% regularization can prevent overfitting
% consistency regularization has been seen as a way to use unlabelled data to aid this process

% distillation also improves performance

% label smoothing also improves performance

%

==> 2_abs_neel.tex <==
%
\begin{abstract}
% The abstract should briefly summarize the contents of the paper in 15--250 words.
Label ambiguity in image segmentation training datasets aggravates the miscalibration of neural networks. As a first contribution, we show that logit consistency across stochastic intensity transformations and geometric deformations acts as an implicit spatially varying regularizer. This regularizer prevents overly confident predictions at pixels with ambiguous labels. As a second contribution, we propose a boundary-weighted extension of this regularizer that provides state-of-the-art calibration for the segmentation of prostate and heart MRI.
\keywords{calibration, consistency regularization, segmentation}
\end{abstract}

==> 3_intro_v2.tex <==
% =========================================================
% Introduction
% =========================================================
\section{Introduction}~\label{sec_intro}

% learning from small datasets is a problem in medical image segmentation
% label ambiguity is another problem
% we would like to have 

% Which of the following is the main point of the paper:
% 1. Why does logit consistency improve network calibration?
% 2. A method to improve network calibration.

% Maybe you should tell the story like this:
% 1. ground truth labels may be ambiguous, having estimates of this ambiguity is difficult, getting multiple labels is difficult
% 2. networks produce over-confident solutions
% 3. we would like to improve calibration - this is the main goal of the paper.
% 4. In particular, becoming over-confident in small dataset regime can be seen as a form of over-fitting (potray this as a special case)

% 5. existing methods for calibration fail to take into account image information

% a problem that is considered independently is that of small datasets -> data augmentation -> consistency reg

% we observe that CR improves calibration even in absense of unlabeled data

% then the explanation for this

% then the proposed extension

\noindent 
Boundaries between anatomical regions are often ambiguous in medical images due to presence of image noise or absence of sufficient contrast.
This issue may be exacerbated by partial volume effects \cite{tohka2014partial}.
Additionally, annotations from multiple clinical experts exhibit substantial variability \cite{becker2019variability}, leading to further ambiguity in what can be considered as \emph{ground truth} labels \cite{jacob2021disentangling}.

==> 4_related_neel.tex <==
\section{Related Work}~\label{sec_related}
\noindent \textbf{Label ambiguity in medical image segmentation} is tackled either by generating multiple plausible segmentations for each image \cite{baumgartner2019phiseg,kohl2018probabilistic}, or by predicting a single well-calibrated segmentation \cite{mehrtash2020confidence} \cite{hong2021hypernet} \cite{islam2021spatially} \cite{larrazabal2021maximum} \cite{murugesan2022calibrating}.
In the latter group, predictions of multiple models are averaged to produce the final segmentation \cite{mehrtash2020confidence} \cite{hong2021hypernet}.
Alternatively, the training loss of a single model is modified to prevent low-entropy predictions at all pixels \cite{murugesan2022calibrating}, at pixels with high errors \cite{larrazabal2021maximum}, and at pixels near boundaries \cite{islam2021spatially}.
Smoothing ground truth labels of pixels only based on distance from boundaries \cite{islam2021spatially} disregards image intensities that cause label ambiguity.
In contrast, the boundary-weighted aspect of our approach emphasizes regularization in those regions but allows the degree of consistency across stochastic transformations to distinguish sub-regions with varying label ambiguity.
On another note, boundary-weighted losses have been proposed for several segmentation contexts \cite{hoopes2022synthstrip} \cite{abulnaga2022automatic}.

\vspace{2pt} \noindent \textbf{Aleatoric uncertainty estimation} in medical images \cite{wang2019aleatoric} \cite{monteiro2020stochastic} is closely related to the problem of pixel-wise label ambiguity due to uncertainty in the underlying image intensities.
While employing stochastic transformations during inference has been shown to produce estimates of aleatoric uncertainty \cite{wang2019aleatoric}, we use them during training to automatically identify regions with ambiguous labels and prevent low-entropy segmentation predictions there.
% \cite{kirchhof2023probabilistic}

\vspace{2pt} \noindent In \textbf{semi-supervised medical image segmentation}, consistency regularization (CR) is widely used \cite{cui2019semi} \cite{bortsova2019semi} \cite{li2020transformation} \cite{wu2022mutual} \cite{luo2022semi} as a means for leveraging unlabelled images to improve absolute segmentation performance.
In contrast, we investigate the capabilities of CR to improve calibration without using any unlabelled images.

\vspace{2pt} \noindent Finally, for \textbf{image classification}, \cite{englesson2021generalized} shows that CR helps mitigate label noise and \cite{muller2019does} employs label smoothing for improving calibration. To our knowledge, this paper is the first to show the role of CR as a means to improve the calibration of segmentation models.

==> 6_exps_part3_old.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{|c|ccc|c|c|cccc|c|c|}
        \hline
        \rowcolor[gray]{0.85}
        Method & \multicolumn{5}{c|}{NCI} & \multicolumn{6}{c|}{ACDC} \\

        \hline
        \rowcolor[gray]{0.9}
        & \multicolumn{3}{c|}{Dice} & ECE & TACE & \multicolumn{4}{c|}{Dice} & ECE & TACE \\

        \rowcolor[gray]{0.9}
        & PZ & CG & Mean &  & & RV & MY & LV & Mean & & \\

        \hline
        \rowcolor[gray]{0.95}
        Baseline &
        43$\pm$23 & 67$\pm$14 & 55$\pm$16 & 41$\pm$16 & 15$\pm$4 &
        48$\pm$21 & 57$\pm$13 & 70$\pm$20 & 58$\pm$15 & 37$\pm$17 & 19$\pm$7 \\

        \rowcolor[gray]{0.95}
        DA \cite{zhang2020generalizing} &
        \textbf{54$\pm$21} & 78$\pm$10 & 66$\pm$13 & 24$\pm$12 & 11$\pm$4 &
        69$\pm$21 & 73$\pm$10 & \textbf{85$\pm$11} & \textbf{76$\pm$12} & 20$\pm$14 & 10$\pm$4 \\

        \rowcolor[gray]{0.95}
        SVLS \cite{islam2021spatially} &
        \textbf{54$\pm$21} & 78$\pm$10 & 66$\pm$14 & 23$\pm$14 & 11$\pm$4 &
        68$\pm$22 & \textbf{73$\pm$9} & \textbf{85$\pm$11} & 75$\pm$12 & 19$\pm$14 & 8$\pm$4 \\

        \rowcolor[gray]{0.95}
        Margin \cite{murugesan2022calibrating} &
        53$\pm$21 & 78$\pm$11 & 66$\pm$14 & 31$\pm$16 & 13$\pm$5 &
        68$\pm$23 & 73$\pm$10 & 85$\pm$12 & 75$\pm$12 & 20$\pm$14 & 10$\pm$4 \\

        \rowcolor[gray]{0.95}
        CR \cite{li2020transformation} &
        51$\pm$21 & 79$\pm$11 & 65$\pm$14 & 18$\pm$14 & 6$\pm$3 &
        68$\pm$22 & 70$\pm$10 & \textbf{85$\pm$11} & 75$\pm$12 & 13$\pm$12 & \textbf{5$\pm$1} \\
        
        \rowcolor[gray]{0.95}
        CR-BW (Ours) &
        \textbf{54$\pm$21} & \textbf{79$\pm$10} & \textbf{67$\pm$13} & \textbf{14$\pm$12} & \textbf{5$\pm$3} & 
        \textbf{70$\pm$21} & 71$\pm$10 & 85$\pm$12 & 75$\pm$11 & \textbf{11$\pm$10} & \textbf{5$\pm$1} \\

        \hline
        
    \end{tabular}

    \vspace{5pt}
    
    \begin{tabular}{|c|ccc|c|cccc|c|}
        \hline
        \rowcolor[gray]{0.85}
        Method & \multicolumn{4}{c|}{NCI} & \multicolumn{5}{c|}{ACDC} \\

        \hline
        \rowcolor[gray]{0.9}
        & \multicolumn{3}{c|}{Dice} & ECE & \multicolumn{4}{c|}{Dice} & ECE \\

        \rowcolor[gray]{0.9}
        & PZ & CG & Mean &  & RV & MY & LV & Mean &  \\

        \hline
        \rowcolor[gray]{0.95}
        Baseline &
        46$\pm$24 & 70$\pm$14 & 58$\pm$17 & 39$\pm$16 &
        60$\pm$22 & 65$\pm$15 & 76$\pm$18 & 67$\pm$15 & 22$\pm$13 \\

        \rowcolor[gray]{0.95}
        DA \cite{zhang2020generalizing} &
        \textbf{57$\pm$22} & 80$\pm$10 & \textbf{69$\pm$13} & 23$\pm$12 &
        80$\pm$14 & 79$\pm$7 & 88$\pm$11 & 82$\pm$8 & 11$\pm$9 \\

        \rowcolor[gray]{0.95}
        SVLS \cite{islam2021spatially} &
        57$\pm$23 & 80$\pm$10 & 69$\pm$14 & 20$\pm$11 &
        \textbf{81$\pm$14} & \textbf{80$\pm$6} & \textbf{88$\pm$10} & \textbf{83$\pm$7} & 9$\pm$8 \\

        \rowcolor[gray]{0.95}
        Margin \cite{murugesan2022calibrating} &
        \textbf{57$\pm$22} & 80$\pm$10 & 68$\pm$14 & 22$\pm$13 &
        80$\pm$15 & 79$\pm$6 & \textbf{88$\pm$10} & 82$\pm$8 & 12$\pm$9 \\

        \rowcolor[gray]{0.95}
        CR \cite{li2020transformation} &
        55$\pm$23 & 80$\pm$11 & 68$\pm$14 & 18$\pm$14 &
        80$\pm$14 & 77$\pm$7 & 87$\pm$10 & 81$\pm$8 & 8$\pm$6 \\
        
        \rowcolor[gray]{0.95}
        CR-BW (Ours) &
        \textbf{57$\pm$22} & \textbf{81$\pm$10} & \textbf{69$\pm$13} & \textbf{13$\pm$12} &
        \textbf{81$\pm$14} & 78$\pm$6 & \textbf{88$\pm$10} & 82$\pm$8 & \textbf{8$\pm$5} \\

        \hline
        
    \end{tabular}

    \vspace{5pt}
    
    \begin{tabular}{|c|ccc|c|cccc|c|}
        \hline
        \rowcolor[gray]{0.85}
        Method & \multicolumn{4}{c|}{NCI} & \multicolumn{5}{c|}{ACDC} \\

        \hline
        \rowcolor[gray]{0.9}
        & \multicolumn{3}{c|}{Dice} & ECE & \multicolumn{4}{c|}{Dice} & ECE \\

        \rowcolor[gray]{0.9}
        & PZ & CG & Mean &  & RV & MY & LV & Mean &  \\

        \hline
        \rowcolor[gray]{0.95}
        Baseline &
        57$\pm$22 & 80$\pm$9 & 68$\pm$13 & 27$\pm$11 &
        85$\pm$11 & 84$\pm$4 & 90$\pm$8 & 86$\pm$6 & 8$\pm$6 \\

        \rowcolor[gray]{0.95}
        DA \cite{zhang2020generalizing} &
        \textbf{66$\pm$19} & \textbf{84$\pm$8} & \textbf{75$\pm$11} & 13$\pm$9 &
        89$\pm$7 & \textbf{87$\pm$3} & 93$\pm$6 & \textbf{90$\pm$3} & 4$\pm$3 \\

        \rowcolor[gray]{0.95}
        SVLS \cite{islam2021spatially} &
        65$\pm$20 & \textbf{84$\pm$8} & 75$\pm$12 & 14$\pm$9 &
        \textbf{90$\pm$6} & \textbf{87$\pm$3} & 93$\pm$6 & \textbf{90$\pm$3} & \textbf{3$\pm$3} \\

        \rowcolor[gray]{0.95}
        Margin \cite{murugesan2022calibrating} &
        65$\pm$21 & \textbf{84$\pm$8} & 75$\pm$12 & 14$\pm$10 &
        90$\pm$7 & \textbf{87$\pm$3} & \textbf{93$\pm$5} & \textbf{90$\pm$3} & \textbf{3$\pm$3} \\

        \rowcolor[gray]{0.95}
        CR \cite{li2020transformation} &
        62$\pm$22 & 84$\pm$9 & 73$\pm$12 & 9$\pm$9 &
        88$\pm$7 & 85$\pm$3 & 92$\pm$6 & 88$\pm$4 & 7$\pm$2 \\
        
        \rowcolor[gray]{0.95}
        CR-BW (Ours) &
        65$\pm$20 & \textbf{84$\pm$8} & \textbf{75$\pm$11} & \textbf{7$\pm$7} &
        89$\pm$6 & 85$\pm$3 & 92$\pm$6 & 89$\pm$3 & 8$\pm$2 \\

        \hline
        
    \end{tabular}
    
    \caption{Results in setting s$1$ (top), s$2$ (middle) and s$3$ (bottom).
    Dice scores and expected calibration errors are reported as 100 * $\mu$ $\pm$ 100 * $\sigma$, where $\mu$ and $\sigma$ are means and standard deviations over all test volumetric images and three experiment runs.}
    \label{tab:example}
\end{table}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\textwidth, trim={0cm 3.25cm 0cm 3.25cm},clip]{figs/subjectwise_ece.png}
    \caption{Subject-wise ECE for NCI (left) and ACDC (right) test subjects, arranged in decreasing order of CR ECE. It can be seen that for most subjects, CR provides better calibration than DA, and boundary-weighted CR provides better calibration than CR. (Figure to be re-generated.)}
    \label{fig_subjectwise_ECE}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\textwidth, trim={0cm 1cm 5cm 0cm},clip]{figs/qualitative_nci_cv1.png}
    \includegraphics[width=0.99\textwidth, trim={0cm 2.75cm 0cm 0cm},clip]{figs/qualitative_acdc_cv1.png}
    \caption{Qualitative comparison of segmentation accuracy and calibration for NCI (top) and ACDC (bottom). Shown subjects are 10th, 50th and 90th percentile of ECE of BW-CR. In each sub-figure, top row shows images and ground truth labels, while following rows show hard predictions and class wise probabilities given by different methods.}
    \label{fig_subjectwise_ECE}
\end{figure}

\begin{table}[t]
    \centering
    \begin{tabular}{|c|ccc|c|cccc|c|}
        \hline
        \rowcolor[gray]{0.85}
        Method & \multicolumn{4}{c|}{NCI} & \multicolumn{5}{c|}{ACDC} \\

        \hline
        \rowcolor[gray]{0.9}
        & \multicolumn{3}{c|}{Dice} & ECE & \multicolumn{4}{c|}{Dice} & ECE \\

        \rowcolor[gray]{0.9}
        & PZ & CG & Mean &  & RV & MY & LV & Mean &  \\

        \hline

        \rowcolor[gray]{0.95}
        CR \cite{li2020transformation} ($\lambda = 0.01$) &
        54$\pm$21 & 79$\pm$10 & 66$\pm$13 & 24$\pm$12 &
        69$\pm$22 & \textbf{72$\pm$10} & 85$\pm$12 & 75$\pm$13 & 19$\pm$14 \\

        \rowcolor[gray]{0.95}
        CR \cite{li2020transformation} ($\lambda = 0.1$) &
        54$\pm$21 & 79$\pm$10 & 66$\pm$13 & 23$\pm$13 &
        68$\pm$23 & \textbf{72$\pm$10} & 85$\pm$12 & 75$\pm$12 & 17$\pm$14 \\

        \rowcolor[gray]{0.95}
        CR \cite{li2020transformation} ($\lambda = 1.0$) &
        52$\pm$21 & 79$\pm$10 & 66$\pm$13 & 17$\pm$12 &
        68$\pm$22 & 70$\pm$10 & \textbf{85$\pm$11} & 75$\pm$12 & 13$\pm$12 \\

        \rowcolor[gray]{0.95}
        CR \cite{li2020transformation} ($\lambda = 10.0$) &
        49$\pm$20 & 78$\pm$11 & 64$\pm$13 & \textbf{13$\pm$11} &
        64$\pm$22 & 63$\pm$12 & 83$\pm$12 & 70$\pm$12 & 16$\pm$11 \\
        
        \rowcolor[gray]{0.95}
        CR-BW (Ours) &
        \textbf{55$\pm$21} & \textbf{79$\pm$9} & \textbf{67$\pm$13} & 14$\pm$11 &
        \textbf{70$\pm$21} & 71$\pm$10 & 85$\pm$12 & \textbf{75$\pm$11} & \textbf{11$\pm$10} \\

        \hline
        
    \end{tabular}
    
    \caption{Effect of $\lambda$ on CR. It can be seen that increasing $\lambda$ in CR improves calibration, but can hurt segmentation accuracy, while CR-BW provides improved calibration as well as equivalent or improved segmentation accuracy.}
    \label{tab:example}
\end{table}
